When is Approximate Counting for Conjunctive Queries Tractable?

Conjunctive queries are one of the most common class of queries used in database systems, and the best studied in the literature. A seminal result of Grohe, Schwentick, and Segoufin (STOC 2001) demonstrates that for every class $G$ of graphs, the evaluation of all conjunctive queries whose underlying graph is in $G$ is tractable if, and only if, $G$ has bounded treewidth. In this work, we extend this characterization to the counting problem for conjunctive queries. Specifically, for every class $C$ of conjunctive queries with bounded treewidth, we introduce the first fully polynomial-time randomized approximation scheme (FPRAS) for counting answers to a query in $C$, and the first polynomial-time algorithm for sampling answers uniformly from a query in $C$. As a corollary, it follows that for every class $G$ of graphs, the counting problem for conjunctive queries whose underlying graph is in $G$ admits an FPRAS if, and only if, $G$ has bounded treewidth (unless $\text{BPP} \neq \text{P}$)}. In fact, our FPRAS is more general, and also applies to conjunctive queries with bounded hypertree width, as well as unions of such queries. The key ingredient in our proof is the resolution of a fundamental counting problem from automata theory. Specifically, we demonstrate the first FPRAS and polynomial time sampler for the set of trees of size $n$ accepted by a tree automaton, which improves the prior quasi-polynomial time randomized approximation scheme (QPRAS) and sampling algorithm of Gore, Jerrum, Kannan, Sweedyk, and Mahaney '97. We demonstrate how this algorithm can be used to obtain an FPRAS for many hitherto open problems, such as counting solutions to constraint satisfaction problems (CSP) with bounded hypertree-width, counting the number of error threads in programs with nested call subroutines, and counting valid assignments to structured DNNF circuits.

==> applications-old.tex <==
% !TeX spellcheck = en_US
%!TEX root = main.tex

\subsection{Constraint satisfaction problems}
\label{sec-csp}
Constraint satisfaction problems offer a general and natural setting to represent a large number of problems where solutions must satisfy some constraints, and which can be found in different areas such as artificial intelligence, satisfiability, programming languages, temporal reasoning, scheduling, graph theory, and databases~\cite{V00,DBLP:books/daglib/0004131,rossi2006handbook,DBLP:books/daglib/0013017,DBLP:series/faia/2009-185,russell2016artificial}. Formally, a constraint satisfaction problem (CSP) is a triple $\cP = (V,D,C)$ such that $V = \{x_1, \ldots, x_m\}$ is a set of variables, $D$ is a set of values and $C = \{C_1, \ldots, C_n\}$ is a set of constraints, where each constraint $C_i$ is a pair $(\bar t_i,R_i)$ such that 
$\bar t_i$ is a tuple of variables from $V$ of arity $k$, for some $k \geq 1$, and $R_i \subseteq D^k$. Moreover, an assignment $\nu : V \to D$ is said to be a solution for $\cP$ if for every $i \in [n]$, it holds that $\nu(\bar t_i) \in R_i$~\cite{russell2016artificial}, where $\nu(\bar t_i)$ is obtained by replacing each variable $x_j$ occurring in $\bar t_i$ by $\nu(x_j)$. The set of solution for CSP $\cP$ is denoted by $\sol(\cP)$. 

The two most basic tasks associated to a CSP are the evaluation and the satisfiability problems. In the evaluation problem, we are given a CSP $\cP$ and an assignment $\nu$, and the question to answer is whether $\nu \in \sol(\cP)$. In the satisfiability problem, we are given a CSP $\cP$, and the question to answer is whether $\sol(\cP) \neq \emptyset$. Clearly, these two problems have very different complexities, as in the former we only need to verify the simple condition that $\nu(t) \in R$ for every constraint $(t,R)$ in $\cP$, while in the latter we need to search in the space of all possible assignments for one that satisfies all the constraints. In fact, these two problems also look  different in terms of our interest in the specific values for the variables of the CSP; in the former we are interested in the value of each one of them that is given in the assignment $\nu$, while in the latter the variables of $\cP$ are considered as existential quantifiers, as we are interested in knowing whether there exists a solution for $\cP$ even if we do not know how to construct it.
As a way to unify these two problems, and to indicate for which variables we are interested in their values, a projection operator has been used in the definition of CSPs~\cite{CJ06,W10}. Notice that the definition of this operator has also played an important role when classifying the complexity of CSPs in terms of algebraic properties of relations~\cite{CJ06}. Formally, an {\em existential} CSP (ECSP) is defined as a pair $\cE = (U, \cP)$, where $\cP = (V,D,C)$ is a CSP and $U \subseteq V$. 
%$V$ is the set of variables of a CSP $\cP$ and $U \subseteq V$, then $\cE = (U, \cP)$ is an {\em existential} CSP (ECSP) whose solutions are defined as follows:
Moreover, the set of solution for $\cE$ is defined as
\begin{eqnarray*}
\sol(\cE) & = & \{ \nu|_{U} \mid \nu \in \sol(\cP)\},
\end{eqnarray*}
where $\nu|_U$ is the restriction of function $\nu$ to the domain $U$. Notice that both the evaluation and the satisfiability problems for a CSP $\cP$ can be reduced to the evaluation problem for an ECSP.
In fact, the satisfiability problem for $\cP$ corresponds to the problem of verifying whether the assignment with empty domain belongs to $\sol(\cE)$, where $\cE$  is the ECSP $(\emptyset, \cP)$.
%, while the problem of checking whether $\nu \in \sol(\cP)$ corresponds to the problem of verifying whether $\nu \in \sol(\cE_2)$ with $\cE_2 = (V, \cP)$. 
Moreover, the evaluation and satisfiability problems are polynomially interreducible for ECSPs, so ECSPs provide a uniform framework for these two problems allowing us to focus only on the evaluation problem.
%In the rest of this section, we focus on the 
% ECSPs provide a uniform framework for both the satisfiability and the evaluation problems for CSPs; in fact, these two problems are polynomially interreducible for ECSPs. 


Clearly the satisfiability problem for CSPs, as well as the evaluation problem for ECSPs, is $\np$-complete; in particular, $\np$-hardness is a consequence that the satisfiability of 3-CNF propositional formulae can be easily encoded as a constraint satisfaction problem. Thus, a large body of research has been devoted to understanding the complexity of the evaluation problem for ECSPs, and finding tractable cases. In particular, two prominent approaches in this investigation have been based on the idea of viewing an ECSP as a homomorphism problem where the target structure is fixed~\cite{FV98,B17,Z17} or on the use of decomposition methods that require of some acyclicity conditions on an ECSP to be satisfied~\cite{GLS00,GLS02}. In this section, we focus on the latter class of methods, and show how the main results of this article can be used to deal with the fundamental problem of counting the number of solutions to an~ECSP. 

\subsubsection{A first notion of acyclicicty}
\label{sec-csp-acyclic}
To define the first notion of acyclicity for ECSPs considered in this article, we need to introduce some terminology. Assume that $\cP = (V,D,C)$ is a CSP such that $V = \{x_1, \ldots, x_m\}$, $C = \{C_1, \ldots, C_n\}$ and $C_i = (\bar t_i, R_i)$ for every $i \in [n]$. Moreover, assume that $\var(\bar t_i)$ is the set of variables mentioned in $\bar t_i$, for every $i \in [n]$. A join tree $T = (N,E)$ for $\cP$ is a rooted tree such that $N = \{\bar t_1, \ldots, \bar t_n\}$, and which satisfies the following connectedness condition:
\begin{itemize}
\item for every $x \in V$, the set $\{ \bar t_i \mid i \in [n]$ and $x \in \var(\bar t_i)\}$ induces a (connected) subtree of $T$.
\end{itemize}
Notice that definition of the notion of join tree does not take into consideration the set $D$ of possible values for the variables, and the relations $R_i$'s used in the definition of the constraints $C_1$, $\ldots$, $C_n$. 
As shown in the following example, some CSPs admit join trees, while others do not. 
\begin{example}\label{exa-join-tree-csp}
Consider a CSP $\cP_1$ with a set of variables $\{u,v,w,x,y\}$ and a set of constraints $\{ C_1, \ldots, C_6\}$ such that each $C_{i} = (\bar t_{i}, R_{i})$, $\bar t_1 = (x,u,v)$, $\bar t_{2} = (x,v,w)$, $\bar t_{3} = (u,y,u)$, $\bar t_{4} = (u,y)$, $\bar t_{5} = (v,w)$ and $\bar t_{6} = (x,y,u)$. Then the following is a join tree $T$ for~$\cP_1$:
\begin{center}
\begin{tikzpicture}
\node[rect] (a1) {$\bar t_{1} = (x,u,v)$};
\node[rectw, below=10mm of a1] (a2) {};
\node[rect, left=9mm of a2] (a3) {$\bar t_{6} = (x,y,u)$}
edge[arrin] (a1);
\node[rect, right=9mm of a2] (a4) {$\bar t_{2} = (x,v,w)$}
edge[arrin] (a1);
\node[rectw, below=10mm of a3] (a5) {};
\node[rect, left=7mm of a5] (a6) {$\bar t_{3} = (u,y,u)$}
edge[arrin] (a3);
\node[rect, right=7mm of a5] (a7) {$\bar t_{4} = (u,y)$}
edge[arrin] (a3);
\node[rect, below=8mm of a4] (a8) {$\bar t_{5} = (v,w)$}
edge[arrin] (a4);
\end{tikzpicture}
\end{center}
Notice that the connectedness condition is satisfied for every variable in the set $\{u,v,w,x,y\}$. For example, the set of atoms mentioning variable $y$ is $\{\bar t_{3}, \bar t_{4}, \bar t_{6}\}$, and this set induces a (connected) subtree of $T$:
\begin{center}
\begin{tikzpicture}
\node[rect] (a3) {$\bar t_{6}$};
\node[rectw, below=10mm of a3] (a5) {};
\node[rect, left=7mm of a5] (a6) {$\bar t_{3}$}
edge[arrin] (a3);
\node[rect, right=7mm of a5] (a7) {$\bar t_{4}$}
edge[arrin] (a3);
\end{tikzpicture}
\end{center}
On the other hand, assume that $\cP_2$ is a CSP with a set of variables $\{x,y,z,w\}$ and a set of constraints $\{ C'_{1}, \ldots, C'_{4}\}$ such that each $C'_{i} = (\bar t'_{i}, R'_{i})$, $\bar t'_{1} = (x,y)$, $\bar t'_{2} = (y,z)$, $\bar t'_{3} = (z,w)$ and $\bar t'_{4} = (w,x)$. Then we have that $\cP_2$ does not admit a join tree. \qed
%\begin{eqnarray*}
%Q_4(x) & \leftarrow & P(x,y),P(y,z),P(z,w),P(w,x).
%\end{eqnarray*}\qed
\end{example}
A CSP $\cP$ is {\em acyclic} if and only if $\cP$ admits a join tree~\cite{Y81,GLS00}. For instance, in Example~\ref{exa-join-tree-csp}, we have that CSP $\cP_1$ is acyclic, while CSP $\cP_2$ is not acyclic. Intuitively, this latter problem is not acyclic as it encodes a cycle of length four. Moreover, an ECSP $(U, \cP)$ is acyclic if and only if $\cP$ is an acyclic CSP. 
 
The notion of acyclic CSP coincides with the notion of $\alpha$-acyclicity for hypergraphs~\cite{F83,BFMY83}, and it has played an important role in finding tractable cases for ECSPs~\cite{GLS00}. In fact, if $\aecsp = \{ (\cE,\nu) \mid \cE$ is an acyclic ECSP and $\nu \in \sol(\cE)\}$, then it holds that \aecsp\ is \logcfl-complete under many-to-one logspace reductions~\cite{GLS98}. Recall that \logcfl\ consists of all decision problems that are logspace reducible to a context-free language, and it holds that $\nlog \subseteq \logcfl \subseteq \acone$. Thus, we have that all problems in \logcfl\ can be solved in polynomial time and are highly parallelizable. 

Concerning to our investigation, we are interested in the fundamental problem of counting the number of solutions to an ECSP. In the most general version of this problem, and even if we focus on CSPs, such a problem is $\sharpp$-complete and cannot admit an FPRAS (unless $\np = \rp$, given that the satisfiability problems for CSP and ECSP are both $\np$-complete). Thus, in this section we focus on this counting problem for acyclic ECSPs:
\begin{center}
	\framebox{
		\begin{tabular}{ll}
			\textbf{Problem:} &  $\saecsp$\\
			\textbf{Input:} & An acyclic ECSP $\cE$\\
			\textbf{Output:} & $|\sol(\cE)|$
		\end{tabular}
	}
\end{center}
It has been shown that $\saecsp$ can be solve in polynomial time if we focus on CSPs, that is, if we focus on ECSPs of the form $(V,\cP)$ where $V$ is the set of variables of $\cP$~\cite{PS13}. However, in the general case we have that \saecsp\ is \sharpp-complete~\cite{PS13}. Thus, a natural and important question is whether \saecsp\ admits an FPRAS. By using the existence of an FPRAS for $\sta$ (see Corollary \ref{cor:fpras-ta-bta}), we are able to give a positive answer to this question. 

\begin{proposition}\label{prop:aecsp}
\saecsp\ admits an FPRAS.
\end{proposition}
\begin{sloppypar}
This proposition can be proved by providing a polynomial-time parsimonious reduction from $\saecsp$ to $\sta$, as we conclude that \saecsp\ admits an FPRAS from the fact that \sta\ admits an FPRAS.
However, as shown in Section \ref{sec-k-hw-ecsp}, Proposition \ref{prop:aecsp} is a corollary of Proposition \ref{prop:skhwecsp}, so we only provide here an intuitive explanation of how the parsimonious reduction from \saecsp\ to \sta\ works.
\end{sloppypar}

Assume that $\cE_1 = (\{x,y\}, \cP_1)$ is an acyclic ECSP, where $\cP_1$ is the acyclic CSP defined in Example~\ref{exa-join-tree-csp}. We first notice that it is proved in~\cite{GLS98} that a canonical join tree for an acyclic CSP can be constructed by a logarithmic space Turing Machine with oracle in $\slog$ (Symmetric Logspace~\cite{LP82}). Thus, given that $\slog = \dlog$~\cite{R08}, it is possible to conclude that a canonical join tree for an acyclic CSP can be constructed in logarithmic space. Hence, the join tree for $\cP_1$ in Example~\ref{exa-join-tree-csp} can be considered as the starting point to show how the reduction from $\saecsp$ to $\sta$ is defined. 

%Recall that $x$ and $y$ are the output variables of $Q_3$, which is highlighted in the following version of the join tree for $Q_3$, where variables $x$ and $y$ are underlined:
%% and we have included the depth for each node in the join tree:
%\begin{center}
%\begin{tikzpicture}
%\node[rect] (a1) {$P(\underline{x},u,v)$};
%\node[rectw, below=10mm of a1] (a2) {};
%\node[rect, left=9mm of a2] (a3) {$R(\underline{x},\underline{y},u)$}
%edge[arrin] (a1);
%\node[rect, right=9mm of a2] (a4) {$P(\underline{x},v,w)$}
%edge[arrin] (a1);
%\node[rectw, below=10mm of a3] (a5) {};
%\node[rect, left=7mm of a5] (a6) {$R(u,\underline{y},u)$}
%edge[arrin] (a3);
%\node[rect, right=7mm of a5] (a7) {$O(u,\underline{y})$}
%edge[arrin] (a3);
%\node[rect, below=8mm of a4] (a8) {$O(v,w)$}
%edge[arrin] (a4);
%\end{tikzpicture}
%\end{center}
Given that the join tree for $\cP_1$ in Example \ref{exa-join-tree-csp} has six nodes, our task is to construct a tree automaton $\cT_{\cE_1} = (S,\Sigma,\Delta,S_0)$ such that $|\sol(\cE_1)|$ is equal to $|\{ t \in \cL(\cT_{\cE_1}) \mid |t| = 6\}|$. Notice that in the general form of the reduction for an acyclic ECSP $\cE = (U, \cP)$, the input of $\sta$ will be a tree automaton $\cT_{\cE}$ and a number $n$ given in unary, which will be equal to the number of constraints in $\cP$. Besides, notice that for the sake of presentation, we are assuming that $\cT_{\cE}$ has a set of initial states, instead of a single initial state. Then the set of states $S$ is used to encode the possible assignments to variables according to the nodes in the join tree for $\cE$:
\begin{align*}
&\{[\bar t_1 \sep (a,b,c)] \mid (a,b,c) \in R_1\} \ \cup \ \{[\bar t_6 \sep (a, b, c)] \mid (a,b,c) \in R_6\} \ \cup\\ 
&\{[\bar t_2 \sep (a,b,c)] \mid (a,b,c) \in R_2\} \ \cup \ \{[\bar t_3 \sep (a, b,a)] \mid (a,b,a) \in R_3\} \ \cup\\
&\{[\bar t_4 \sep (a, b)] \mid (a,b) \in R_4\} \ \cup \ \{[\bar t_5 \sep (a, b)] \mid (a,b) \in R_5\}
\end{align*}
Moreover, the set $S_0$ of initial states is defined as the set of possibles assignments for the root of the join tree: $S_0 = \{[\bar t_1 \sep (a,b,c)] \mid (a,b,c) \in R_1 \}$, and the alphabet $\Sigma$ is defined as the set of possibles assignments for the set $\{x,y\}$ of output variables of $\cE$:
\begin{align*}
&\{[\bar t_1 \sep (a,\star,\star)] \mid \exists b \exists c : (a,b,c) \in R_1\} \ \cup \
\{[\bar t_6 \sep (a, b,\star)] \mid \exists c : (a,b,c) \in R_6\} \ \cup\\
&\{[\bar t_2 \sep (a,\star,\star)] \mid \exists b \exists c : (a,b,c) \in R_2\} \ \cup \
\{[\bar t_3 \sep (\star,b,\star)] \mid \exists a : (a,b,a) \in R_3\} \ \cup\\
&\{[\bar t_4 \sep (\star,b)] \mid \exists a : (a,b) \in R_4\}\ \ \cup\ 
\{[\bar t_5 \sep (\star,\star)] \mid \exists a \exists b : (a,b) \in R_5\}
\end{align*}
The symbol $\star$ is used in a position of a tuple if we are not assigning a value for an output variable in such a position. Notice that $S$, $S_0$ and $\Sigma$ can be constructed in polynomial time since they are defined from the relations in the constraints of $\cE_1$. In other words, something that we cannot do in the reduction is to use generic assignments of the from $(x_1, \ldots, x_\ell) \sep (a_1, \ldots, a_\ell)$, where $x_1$, $\ldots$, $x_\ell$ is the sequence of variables from $\cP_1$ and $a_1$, $\ldots$, $a_\ell$ is a sequence of possible values for these variables, as we can have an exponential number of such assignments. Finally, the transition relation $\Delta$ is defined to represent a top-down evaluation of the join tree for the ECSP $\cE$. For instance, if we have that $(a,b,c) \in R_1$, $(a,c,e) \in R_6$ and $(a,d,b) \in R_2$, then the following is a tuple in $\Delta$:
\begin{eqnarray*}
\big([\bar t_1 \sep (a, b, c)], [\bar t_1 \sep (a,\star,\star)], [\bar t_6 \sep (a,d,b)][\bar t_2 \sep (a,c,e)]\big).
\end{eqnarray*}
This tuple indicate that if we are in the state $[\bar t_1 \sep (a, b, c)]$ in the root of the tree and the label of this node is $[\bar t_1 \sep (a,\star,\star)]$, then we assign the states $[\bar t_6 \sep (a,d,b)]$ and $[\bar t_2 \sep (a,c,e)]$ to the left and right children of the root, respectively. That is, this tuple indicates that if $(a,b,c)\in R_1$, then we can assign to $x$ value $a$ according to the root of the join tree, and then given that $(a,d,b) \in R_6$ and $(a,c,e) \in R_2$, we can continue with the computation of a solution for $\cE$ by using the assignments $x\sep a, y\sep d, u\sep b$ and 
$x\sep a, v\sep c, w\sep e$ in the left and right children of the root node. In general, we have that $\Delta$ is the following set:
\begin{align*}[
&\big\{ \big([\bar t_1 \sep (a, b, c)], [\bar t_1 \sep (a,\star,\star)], [\bar t_6 \sep (a,d,b)][\bar t_2 \sep (a,c,e)]\big) \ \big| \\  
&\hspace{200pt}[\bar t_1 \sep (a, b, c)] \in S_0, [\bar t_1 \sep (a,\star,\star)] \in \Sigma,\\
&\hspace{200pt}[\bar t_6 \sep (a,d,b)] \in S \text{ and } [\bar t_2 \sep (a,c,e)] \in S \big\} \ \cup\\
&\big\{ \big([\bar t_6 \sep (a, b, c)], [\bar t_6 \to (a,b,\star)], [\bar t_3 \sep (c, b, c)][\bar t_4 \sep (c, b)]\big) \ \big|\\
&\hspace{213pt}[\bar t_6 \sep (a, b, c)] \in S, [\bar t_6 \to (a,b,\star)] \in \Sigma\\
&\hspace{213pt}[\bar t_3 \sep (c, b, c)] \in S \text{ and } [\bar t_4 \sep (c, b)] \in S \big\}\ \cup\\
&\big\{ \big([\bar t_2 \sep (a, b, c)], [\bar t_2 \sep (a,\star,\star)], [\bar t_5 \sep (b,c)]\big) \ \big|\\
&\hspace{119pt} [\bar t_2 \sep (a, b, c)] \in S, [\bar t_2 \sep (a,\star,\star)] \in \Sigma \text{ and } [\bar t_5 \sep (b,c)] \in S\big\} \ \cup\\
&\big\{ \big([\bar t_3 \sep (a, b, a)], [\bar t_3 \sep (\star,b,\star)], \lambda \big) \ \big| \ [\bar t_3 \sep (a, b, a)] \in S \text{ and } [\bar t_3 \sep (\star,b,\star)] \in \Sigma \big\} \ \cup\\
&\big\{ \big([\bar t_4 \sep (a, b)], [\bar t_4 \sep (\star,b)], \lambda \big) \ \big| \ [\bar t_4 \sep (a, b)] \in S \text{ and } [\bar t_4 \sep (\star,b)] \in \Sigma \big\} \ \cup\\
&\big\{ \big([\bar t_5 \sep (a,b)], [\bar t_5 \sep (\star,\star)], \lambda \big) \ \big| \ [\bar t_5 \sep (a,b)] \in S \text{ and } [\bar t_5 \sep (\star,\star)] \in \Sigma \big\}.
\end{align*}
Thus, the transition relation encodes a top-down evaluation of the join tree for ECSP $\cE$. In particular, for each node $p$ and each children $p'$ of $p$ in the join tree, if a variable $z$ is mentioned in both, then its value is inherited from $p$ to $p'$, and if $z$ appears in $p'$ but not in $p$, then its value is guessed. It is important to notice that we have a consistent way of assigning values to the variables of $\cE$ given the inheritance rule just described and the connectedness condition satisfied by the join tree of $\cE$ (that is, it is not possible to assign two different values to the same variable). 

As a final remark, it is important to notice that $\cT_{\cE_1}$ can be constructed in polynomial time, and that each posible solution to $\cE_1$ is associated with exactly with one tree $t$ such that $t$ is accepted  by $\cT_{\cE_1}$ and $|t| = 6$. In particular, observe that all trees accepted by $\cT_{\cE_1}$ have six nodes by definition of this automaton.  For example, assuming that $\nu(x) = a $ and $\nu(b) = b$ is an assignment such that $\nu \in \sol(\cE_1)$, we have that the following tree accepted by $\cT_{\cE_1}$ is associated to $\nu$:
\begin{center}
\begin{tikzpicture}
\node[rect] (a1) {$[\bar t_1 \sep (a,\star,\star)]$};
\node[rectw, below=10mm of a1] (a2) {};
\node[rect, left=12mm of a2] (a3) {$[\bar t_6 \to (a,b,\star)]$}
edge[arrin] (a1);
\node[rect, right=12mm of a2] (a4) {$[\bar t_2 \sep (a,\star,\star)]$}
edge[arrin] (a1);
\node[rectw, below=10mm of a3] (a5) {};
\node[rect, left=7mm of a5] (a6) {$[\bar t_3 \sep (\star,b,\star)]$}
edge[arrin] (a3);
\node[rect, right=7mm of a5] (a7) {$[\bar t_4 \sep (\star,b)]$}
edge[arrin] (a3);
\node[rect, below=8mm of a4] (a8) {$[\bar t_5 \sep (\star,\star)]$}
edge[arrin] (a4);
\end{tikzpicture}
\end{center}
Hence, we conclude that the reduction from $\saecsp$ to $\sta$ just described is a parsimonious reduction that can be computed in polynomial time. 

\subsubsection{A more general notion of acyclicity}
\label{sec-k-hw-ecsp}

In this section, we consider a more general notion of acyclicity for ECSPs. 
More precisely, let $\cP =(V,D,C)$ be a CSP such that $C = \{C_1, \ldots, C_n\}$ and $C_i = (\bar t_i,R_i)$ for each $i \in [n]$. A hypertree for $\cP$ is a triple $\langle T, \chi, \xi\rangle$ such that $T = (N,E)$ is a rooted tree, and $\chi$ and $\xi$  are node-labelling functions such that for every $p \in N$, it holds that $\chi(p) \subseteq V$ and  $\xi(p) \subseteq \{\bar t_1, \ldots, \bar t_n\}$. Moreover, $T$ is said to be a hypertree decomposition for $\cP$~\cite{GLS02} if the following conditions hold:
\begin{itemize}
\item for each atom $i \in [n]$, there exists $p \in N$ such that $\var(\bar t_i) \subseteq \chi(p)$;

\item for each variable $x \in V$, the set $\{ p \in N \mid x \in \chi(p)\}$ induces a (connected) subtree of $T$;

\item for each $p \in N$, it holds that 
\begin{eqnarray*}
\chi(p) & \subseteq & \bigcup_{\bar t \in \xi(p)} \var(\bar t)
\end{eqnarray*}

\item for each $p \in N$, it holds that
\begin{eqnarray*}
\bigg(\bigcup_{\bar t \in \xi(p)} \var(\bar t)\bigg) \cap \bigg(\bigcup_{p' \,:\, p' \text{ is a descendant of } p \text{ in } T} \chi(p')\bigg) &  \subseteq & \chi(p)
\end{eqnarray*}
\end{itemize}
The width of the hypertree decomposition $\langle T, \chi, \xi\rangle$ is defined as the maximum value of $|\xi(p)|$ over all vertices $p \in N$. Finally, the hypertree-width $\hw(\cP)$ of CSP $\cP$ is defined as the minimum width over all its hypertree decompositions~\cite{GLS02}. 

\begin{example}
Consider again the CSPs $\cP_1$ and $\cP_2$ defined in Example \ref{exa-join-tree-csp}. The following is a hypertree decomposition for $\cP_1$, where the values of $\chi(p)$ and $\xi(p)$ are shown on the left- and right-hand sides of the rectangle for node $p$:
\begin{center}
\begin{tikzpicture}
\node[rect] (a1) {$\{x,u,v\}$, $\{\bar t_1\}$};
\node[rectw, below=10mm of a1] (a2) {};
\node[rect, left=11mm of a2] (a3) {$\{x,y,u\}$, $\{\bar t_6\}$}
edge[arrin] (a1);
\node[rect, right=11mm of a2] (a4) {$\{x,v,w\}$, $\{\bar t_2\}$}
edge[arrin] (a1);
\node[rectw, below=10mm of a3] (a5) {};
\node[rect, left=7mm of a5] (a6) {$\{y,u\}$, $\{\bar t_3\}$}
edge[arrin] (a3);
\node[rect, right=7mm of a5] (a7) {$\{u,y\}$, $\{\bar t_4\}$}
edge[arrin] (a3);
\node[rect, below=8mm of a4] (a8) {$\{v,w\}$, $\{\bar t_5\}$}
edge[arrin] (a4);
\end{tikzpicture}
\end{center}
Notice that the width of this hypertree decomposition is 1, as $|\xi(p)| = 1$ for every node $p$ in it. Thus, we conclude that $\hw(\cP_1) = 1$. On the other hand, no hypertree decomposition of width~1 can be constructed for $\cP_2$. In fact, $\hw(\cP_2) = 2$, which is witnessed by the following hypertree decomposition for $\cP_2$ of width 2:
\begin{center}
\begin{tikzpicture}
\node[rect] (a3) {$\{x,y,z\}$, $\{\bar t'_1,\bar t'_2\}$};
\node[rect, below=8mm of a3] (a5) {$\{x,z,w\}$, $\{\bar t'_3,\bar t'_4\}$}
edge[arrin] (a3);
\end{tikzpicture}
\end{center} \qed
\end{example}
It was shown in \cite{GLS02} that a CSP $\cP$ is acyclic if and only if $\hw(\cP) = 1$. Thus, the notion of hypertree-width generalizes the notion of acyclicity given in the previous section. More importantly, it was shown in \cite{GLS02} that the evaluation problem for ECSPs of bounded hypertree-width can be solved efficiently. More precisely, given an ECSP $\cE = (U,\cP)$, define $\hw(\cE)$ as $\hw(\cP)$, and for $k \geq 1$ define the language $\khwecsp =  \{ (\cE,\nu) \mid \cE$ is an ECSP such that $\hw(\cE) \leq k$ and $\nu \in \sol(\cE)\}$. 
Then it holds that $\khwecsp$ is \logcfl-complete under many-to-one logspace reductions~\cite{GLS02}, which, as mentioned before, implies that $\khwecsp$ can be solved in polynomial time and is highly parallelizable. Concerning to our investigation, we are interested in the following fundamental problem associated to the evaluation problem for $\khwecsp$:
\begin{center}
	\framebox{
		\begin{tabular}{ll}
			\textbf{Problem:} &  $\skhwecsp$\\
			\textbf{Input:} & An ECSP $\cE$ such that $\hw(\cE) \leq k$\\
			\textbf{Output:} & $|\sol(\cE)|$
		\end{tabular}
	}
\end{center}
As for the case of acyclic ECSPs, it was shown in \cite{PS13} that for every $k \geq 1$, the counting problem $\skhwecsp$ is $\sharpp$-complete, and it can be solved in polynomial time if we restrict to the case of CSPs (that is, ECSPs of the form $(V,\cP)$ where $V$ is the set of variables of $\cP$). Thus, a fundamental question is whether $\skhwecsp$ admits an FPRAS. 
%the existence of an FPRAS for acyclic ECSPs can be extended to the case of $\skhwecsp$. 
In the following proposition, we give a positive answer to this question. Notice that from this result we obtain Proposition \ref{prop:aecsp} as a corollary given that $\saecsp = \sohwecsp$.

\begin{proposition}\label{prop:skhwecsp}
For every $k \geq 1$, it holds that \skhwecsp\ admits an FPRAS.
\end{proposition}
The proof of this proposition is given in Appendix \ref{proof:prop:skhwecsp}.

\subsection{Conjunctive queries}
\label{sec-acyclic}
Conjunctive queries are the most common class of queries used in database systems, as well as the most studied in the database literature. They correspond to the Select-Project-Join queries of SQL. Formally, a conjunctive query (CQ) is an expression of the form:
\begin{eqnarray} \label{eq:cq-def}
Q(\bar x)  & \leftarrow & S_1(\bar u_1) \wedge \cdots \wedge S_n(\bar u_n),
\end{eqnarray} 
where for every $i \in [n]$, $S_i$ is a $k$-ary relation symbol and $\bar u_i$ is 
a $k$-ary tuple of variables and constants, and $\bar x$ is a tuple of variables such that each variable in $\bar x$ occurs in some $\bar u_i$.
%, where repetitions are allowed; for instance, we can
%write $R(x,x,y)$ and $O(a,x,a,x)$, where $x,y$ are variables and $a$ is a constant.  
The symbol $Q$ is used as the name of the query.
%, $\atom(Q) = \{S_1(\bar u_1), \cdots, S_n(\bar u_n)\}$, and for each $A \in \atom(Q)$, $\var(A)$ is used to denote the set of variables occurring in $A$, so that $\var(Q)$ is defined as $\var(S_1(\bar u_1)) \cup \cdots \cup \var(S_n(\bar u_n))$. 
Intuitively, the left-hand side $S_1(\bar u_1) \wedge \cdots \wedge S_n(\bar u_n)$ of $Q$ is used to specify a pattern over a database, while the tuple $\bar x$ is used to store the answer to the query when such a pattern is found. More precisely, a database $I$ is a set of facts of the form $T(\bar a)$, which indicates that $\bar a$ is a tuple in the table $T$ in $I$. Then a homomorphism from $Q$ to $I$ is a function from the set of variables occurring in $Q$ to the constants in $I$ such that for every $i \in [1,n]$, it holds that $S_i(h(\bar u_i))$ is a fact in $I$,
%tuple in the table $S_i$ in $I$, 
where $h(\bar u_i)$ is obtained by applying $h$ to each component of $\bar u_i$ leaving the constants unchanged. Moreover, given such a homomorphism $h$, the tuple of constants $h(\bar x)$ is said to be an answer to $Q$ over the database $I$, and $\answer(Q,I)$ is defined as the set of answers of $Q$ over $I$. 
%Again such variables can repeat,
%i.e., we can write $Q(x,x,z) = \exists y\ R(x,x,y) \wedge O(z,x)$. 






 \begin{example}\label{exa-cq-dat}
 Consider a university database consisting of the following relations:  \Enrolled(\sno, \cno) indicates that a student with identifier \sno\ is taking a course with identifier \cno, \Course(\cno, \dno) indicates that a course with identifier \cno\ is given by a department with identifier \dno, and \Dept(\dno, \name) indicates that \name\ is the name of the department with identifier \dno. The following is a simple university database $I$:
 \begin{center}
 \begin{tabular}{c|cc|cc|cc|cc|cc|}\cline{2-3} \cline{6-7} \cline{10-11}
 \Enrolled & \sno & \cno &  & \Course & \cno & \dno & & \Dept & \dno & \name\\ \cline{1-3} \cline{5-7} \cline{9-11}
 & st1 & mat101 & & & cs101 & dept1 & & & dept1 & Computer Science\\
 & st1 & stat101 & & & stat101 & dept3 & & & dept2 & Mathematics\\
 & st2 & mat101 & & & mat101 & dept2 & & & dept3 & Statistics\\\cline{6-7}  \cline{10-11}
 & st2 & cs101\\\cline{2-3}
 \end{tabular}
\end{center}
The following CQ can be used to retrieve the list of students that are taking at least one course:
\begin{eqnarray*}
Q_1(x) &=& \exists y \,  \Enrolled(x,y).
\end{eqnarray*}
In fact, we have that st1 is an answer to $Q_1$ over $I$ since the function $h$ defined as $h(x) = \text{st1}$ and $h(y) = \text{mat101}$ is a homomorphism from $Q_1$ to $I$ such that $h(x) = \text{st1}$; in particular, we have that $h$ is a homomorphism since $\Enrolled(h(x),h(y)) = \Enrolled(\text{st1}, \text{mat101})$ is a fact 
%tuple in the table \Enrolled\ in the database 
in $I$. In the same way, it can be shown that \text{st2} is an answer to $Q_1$ over $I$. In fact, we have that $\answer(Q,I) = \{\text{st1}, \text{st2}\}$. Moreover, the following CQ can be used to retrieve the list of students that are taking at least one course in the Department of Computer Science:
\begin{eqnarray*}
Q_2(x) &=& \exists y \exists z \, \Enrolled(x,y) \wedge \Course(y,z) \wedge \Dept(z,\text{``Computer Science''}).
\end{eqnarray*}
Notice that $Q_2$ includes the constant ``Computer Science''. \qed
 \end{example}
The problem of evaluating a conjunctive query over a database is a fundamental problem that has been widely studied. In its decision version, it can be defined as the problem of verifying, given a CQ $Q$, a database $I$ and a tuple of constants $\bar a$, whether $\bar a$ is an answer to $Q$ over $I$ (that is, whether $\bar a \in \answer(Q,I)$). It is well-known that such a problem is $\np$-complete~\cite{CM77}, so many restrictions ensuring tractability have been explored in the literature~\cite{Y81,CR97,GSS01,GLS02,GGLS16}. In particular, starting with the work in~\cite{Y81}, a line of research that has been particularly fruitful in finding tractable cases is based on analyzing the {\em degree of cyclicity} of the underlying structure of a conjunctive query. 

The evaluation problem for CQs is equivalent to the evaluation problem for  existential CSPs~\cite{KV00}, which are studied in Section \ref{sec-csp}. To see why this is the case, we first notice that we can focus on CQs not mentioning constants, as a constant $a$ in a query $Q$ can always be encoded by adding a fresh table $T_a$ that consists only of the constant $a$, replacing $a$ by a fresh variable $x_a$ in $Q$ and adding to $Q$ an atom $T_a(x_a)$. For instance, to evaluate $Q(x) \leftarrow R(x,a) \wedge O(x,y,a)$ over a database $I$ is equivalent to evaluate CQ $Q'(x) \leftarrow R(x,x_a) \wedge O(x,y,x_a) \wedge T_a(x_a)$ over a database $I'$ constructed by adding to $I$ a table $T_a$ consisting only of the constant $a$. Thus, when showing how to transform a CQ $Q$ and a database $I$ into an ECSP $\cE_{Q,I}$,\footnote{The transformation in the opposite direction is done analogously.} we can assume that $Q$ is of the \eqref{eq:cq-def} but without mentioning any constants. More precisely, we define $\cE_{Q,I} = (U, \cP)$, where $U$ is the set of variables occurring in $\bar x$, $\cP = (V, D,C)$, $V$ is the set of variable occurring in $S_1(\bar u_1) \wedge \cdots \wedge S_n(\bar u_n)$, $D$ is the set of constants occurring in $I$ and $C$ is the following set of constraints. For each $i \in [n]$, define a constraint $C_i = (\bar u_i, R_i)$, where $R_i = \{ \bar a \mid S_i(\bar a)$ is a fact in $I\}$. Moreover, assuming that $\bar x = (x_1, \ldots, x_m)$, and that $\bar a = (a_1, \ldots, a_m)$ is a tuple of constants from $D$ that is consistent with $\bar x$ in the sense that $a_i = a_j$ whenever $x_i = x_j$, define an assignment $\nu_{\bar a}$ as $\nu_{\bar a}(x_i) = a_i$ for every $i \in [m]$. Then it is easy to see that for every tuple $\bar a$ of constants, it holds that:
\begin{eqnarray*}
\bar a \in \answer(Q,I) & \text{ if and only if } & \nu_{\bar a} \in \sol(\cE_{Q,I}).
\end{eqnarray*}
This tight connection can be used to extend the notions of acyclicity  given in Sections \ref{sec-csp-acyclic} and~\ref{sec-k-hw-ecsp} to the case of CQs. More precisely, given a CQ $Q$, notice that by definition of the notions of acyclicity in Section \ref{sec-csp-acyclic} and hypertree-width in Section \ref{sec-k-hw-ecsp}, we have that for every pair of databases $I_1$, $I_2$, it holds that $\cE_{Q,I_1}$ is acyclic if and only if $\cE_{Q,I_2}$ is acyclic, and $\hw(\cE_{Q,I_1}) = \hw(\cE_{Q,I_2})$. Thus, given an arbitrary database $I$, conjunctive query $Q$ is said to be acyclic if and only if $\cE_{Q,I}$ is acyclic~\cite{Y81,GLS98}, and $\hw(Q)$ is defined as $\hw(\cE_{Q,I})$~\cite{GLS02}. 

Concerning to our investigation, we are interested in the fundamental problem of counting the number of answers to a conjunctive query over a database. In general,  this problem is $\sharpp$-complete and cannot admit an FPRAS (unless $\np = \rp$, given that the evaluation problem for CQs is $\np$-complete). Thus, we focus on the following fundamental problems where the degree of cyclicity of conjunctive queries is bounded. 
\begin{center}
\begin{tabular}{c}
	\framebox{
		\begin{tabular}{lp{10.3cm}}
			\textbf{Problem:} &  $\sacq$\\
			\textbf{Input:} & An acyclic conjunctive query $Q$ and a database $I$\\
			\textbf{Output:} & $|\answer(Q,I)|$
		\end{tabular}
	}\\
	\\
	\framebox{
		\begin{tabular}{lp{10.3cm}}
			\textbf{Problem:} &  $\skhw$\\
			\textbf{Input:} & A conjunctive query $Q$ such that $\hw(Q) \leq k$ and a database $I$\\
			\textbf{Output:} & $|\answer(Q,I)|$
		\end{tabular}
	}
\end{tabular}	
\end{center}
It is important to notice that $\sacq = \sohw$, as it is proved in \cite{GLS02} that a CQ is acyclic if and only if $\hw(Q) = 1$. However, we will keep both languages for historical reasons, as acyclic conjunctive queries were defined two decades earlier and are widely used and more popular in databases.
Both $\sacq$ and $\skhw$, for a fixed $k \geq 1$, are known to be $\sharpp$-complete~\cite{PS13}. On the positive side, from the characterization of the evaluation problem of CQs in terms of the evaluation problem for ECSPs and Propositions \ref{prop:aecsp} and \ref{prop:skhwecsp}, we conclude that these problems admit FPRAS.
\begin{proposition}\label{prop:acq-skhw}
\sacq\ admits an FPRAS, and for every $k \geq 1$, $\skhw$ admits an FPRAS.
\end{proposition}

\subsection{Union of conjunctive queries}
An important and well-studied extension of the class of conjunctive queries is obtained by adding the union operator. A union of conjunctive queries (UCQ) is an expression of the form:
\begin{eqnarray}\label{eq:ucq_def}
Q(\bar x) & \leftarrow & Q_1(\bar x) \vee \cdots \vee Q_m(\bar x),
\end{eqnarray}
where $Q_i(\bar x)$ is a conjunctive query for each $i \in [m]$, and the same tuple $\bar x$ of output variables is used in the CQs $Q_1(\bar x)$, $\ldots$, $Q_m(\bar x)$. As for the case of CQs, the symbol $Q$ is used as the name of the query. For instance, if we consider again the CQ $Q_2(x)$ and the database given in Example~\ref{exa-cq-dat}, and if we define $Q_6(x)$ as the following CQ:
\begin{eqnarray*}
Q_6(x) &=& \exists y \exists z \, \Enrolled(x,y) \wedge \Course(y,z) \wedge \Dept(z,\text{``Statistics''}),
\end{eqnarray*}
then the union of conjunctive queries $Q(x) \leftarrow Q_2(x) \vee Q_6(x)$ can be used to retrieve the list of students that are taking at least one course in the Department of Computer Science or in the Department of Statistics. 

A tuple $\bar a$ is said to be an answer of UCQ $Q$ in \eqref{eq:ucq_def} over a database $I$ if and only if $\bar a$ is an answer to $Q_i$ over $I$ for some $i \in [m]$. Thus, we have that:
\begin{eqnarray*}
\answer(Q,I) &=& \bigcup_{i=1}^m \answer(Q_i,I).
\end{eqnarray*} 
As for the case of CQs, without loss of generality we can focus on UCQs without constants. 
As expected, the problem of verifying, given a UCQ $Q$, a database $I$ and a tuple of constants $\bar a$, whether $\bar a$ is an answer to $Q$ over $I$ is an $\np$-complete problem~\cite{CM77}. Also as expected, the evaluation problem for union of acyclic conjunctive queries can be solved in polynomial time, given that the evaluation problem for acyclic CQs can be solved in polynomial time.
Concerning to our investigation, we are interested in the following fundamental problem associated to the evaluation problem for union of acyclic conjunctive queries:
\begin{center}
	\framebox{
		\begin{tabular}{ll}
			\textbf{Problem:} &  $\suacq$\\
			\textbf{Input:} & A union of acyclic conjunctive queries $Q$ and a database $I$\\
			\textbf{Output:} & $|\answer(Q,I)|$
		\end{tabular}
	}
\end{center}
As expected from the result for conjunctive queries, $\suacq$ is \sharpp-complete~\cite{PS13}. However, $\suacq$ remains $\sharpp$-hard even if we focus on the case of UCQs without existentially quantified variables, that is, UCQs of the form \eqref{eq:ucq_def} where $\bar x$ consists of all the variables occurring in CQ $Q_i(\bar x)$ for each $i \in [m]$. Notice that this is in sharp contrast with the case of CQs, where $\sacq$ can be solved in polynomial time if we focus on case of CQs without existentially quantified variables~\cite{PS13}. 
% even when restricted to union of full acyclic conjunctive queries~\cite{PS13}. 
%Unfortunately, the tractability of $\sacq$ for full acyclic CQs does not carry over the union of such queries. More precisely, and in sharp contrast with what was mentioned before, the problem $\suacq$ is \sharpp-complete even when restricted to union of full acyclic conjunctive queries~\cite{PS13}. 
However, by using Proposition \ref{prop:acq-skhw}, we are able to provide a positive result about the possibility of efficiently approximating $\suacq$.
\begin{proposition}\label{prop:uacq}
\suacq\ admits an FPRAS.
\end{proposition}

\begin{proof}
We need to prove that there exists a randomized algorithm $\cA$ and a polynomial $p(x,y)$ such that $\cA$ receives as input a union of acyclic conjunctive queries $Q$, a database $I$ and $\eps \in (0,1)$, $\cA$ works in time $p(\|Q\|+\|I\|,\eps^{-1})$, where $\|Q\|+\|I\|$ is the size of $Q$ and $I$, 
 and $\cA$ satisfies the following condition:
\begin{eqnarray*}
\pr{|\cA(Q,I,\eps) - |\answer(Q,I)|| \leq \eps \cdot |\answer(Q,I)|} & \geq & \frac{3}{4}.
\end{eqnarray*}
Assume that $Q$ is of the form \eqref{eq:ucq_def}, from which we have that $\answer(Q,I) = \bigcup_{i=1}^m \answer(Q_i,I)$ and, therefore, $|\answer(Q,I)| = |\bigcup_{i=1}^m \answer(Q_i,I)|$. Thus, we know from \cite{KL83} that the algorithm $\cA$ can be constructed if three conditions are satisfied: (a) there exists a polynomial-time algorithm that verifies whether $\bar a \in \answer(Q_i,I)$; (b) there exists a randomized polynomial-time algorithm that generates an element in $\answer(Q_i,I)$ with uniform distribution; and (c) there exists a polynomial-time algorithm that computes $|\answer(Q_i,I)|$. In our case, property (a) holds as each $Q_i(\bar x)$ is an acyclic conjunctive query, while condition (c) cannot hold unless $\fp = \sharpp$, given that $\sacq$ is $\sharpp$-complete. However, as shown in \cite{gore1997quasi}, the existence of algorithm $\cA$ can still be guaranteed under condition (a) and the existence of an FPRAS for the function $(Q_i,I) \mapsto |\answer(Q_i,I)|$, as this latter condition also implies the existence of a fully polynomial-time almost uniform generator for $\answer(Q_i,I)$~\cite{JVV86}. Therefore, we conclude that algorithm $\cA$ exists from Proposition \ref{prop:acq-skhw}
\end{proof}

As a final fundamental problem, we consider the problem of counting the number of solutions of a union of conjunctive queries of bounded hypertree-with.
\begin{center}
	\framebox{
		\begin{tabular}{lp{11cm}}
			\textbf{Problem:} &  $\skuhw$\\
			\textbf{Input:} & A union of conjunctive query $Q(\bar x) \leftarrow Q_1(\bar x) \vee \cdots \vee Q_m(\bar x)$ such that $\hw(Q_i) \leq k$ for every $i \in [m]$, and a database $I$\\
			\textbf{Output:} & $|\answer(Q,I)|$
		\end{tabular}
	}
\end{center}
By using the same ideas as in the proof of Proposition \ref{prop:uacq}, we obtain from Proposition \ref{prop:acq-skhw} that:
\begin{proposition}\label{prop:skuhw}
For every $k \geq 1$, it holds that $\skuhw$ admits an FPRAS.
\end{proposition}




\subsection{Nested words}
Nested words have been proposed as a model for the formal verification of correctness of structured programs that can contain nested calls to subroutines~\cite{AEM04,AM04,AM09}. In particular, the execution of a program is viewed as a linear sequence of states, but where a matching relation is used to specify the correspondence between each point during the execution at which a procedure is called with the point when we return from that procedure call. 

Formally, a binary relation $\mu$ on an interval $[n]$ is a matching if the following conditions hold:
(a) if $\mu(i,j)$ holds then $i < j$; 
(b) if $\mu(i,j)$ and $\mu(i,j')$ hold
then $j = j'$, and if $\mu(i,j)$ and $\mu(i',j)$ hold then $i = i'$; 
(c) if $\mu(i,j)$ and $\mu(i',j')$ hold, where $i \neq i'$ and $j \neq j'$, then either $[i,j] \cap [i',j'] = \emptyset$ or $[i,j] \subseteq [i',j']$ or $[i',j'] \subseteq [i,j]$. Moreover, given a finite alphabet $\Sigma$,  a {\em nested word} of length $n$ over $\Sigma$ is a tuple $\w=(w,\mu)$, where
$w \in \Sigma^*$ is a string of length $n$, and $\mu$ is a matching on $[n]$.  





%We say that 
A position $i$ in a nested word 
$\w$ is a call (resp., return) position if there exists $j$ such that $\mu(i,j)$ (resp., $\mu(j,i)$) holds.
If $i$ is neither a call nor a return position in $\w$, then $i$ is said to be an internal position in $\w$. 
%Moreover, if $\mu(i,j)$ holds, we say that $i$ is the matching call of $j$, and $j$ is
%the matching return of $i$.
Figure~\ref{fig:shape} shows a nested word (without the
labeling with alphabet symbols). Solid lines are used to draw the linear edges that define a standard word, while nesting edges are drawn using dashed
lines. Thus, the relation $\mu$ is $\{(2,4), (5,6), (1,7)\}$, the set of call positions is $\{1,2,5\}$, the set of return positions is $\{4,6,7\}$ and the set of internal positions is~$\{3,8\}$.
%Linear edges from call positions are call edges going down, and linear
%edges to returns are return edges going up.  
%Thus, the sequence has a pending call, which is depicted by a dashed outgoing edge.


Properties to be formally verified are specified by using nested word automata. Such automata have the same expressiveness as monadic second order logic over
nested words~\cite{AM09}, so they are expressive enough to allow the specification and automatic verification of a large variety of properties over programs with nested calls to subroutines. 
Formally, a (nondeterministic) {\em nested word automaton} (NWA) $\cN$ 
is a tuple $(S, \Sigma, S_0, F, P, \cd, \id, \rd )$ consisting of
a finite set of states $S$,
an alphabet $\Sigma$, 
a set of initial states $S_0 \subseteq S$,
a set of final states   $F \subseteq S$,
a finite set of hierarchical symbols $P$,
%a set of initial hierarchical symbols $P_0\subseteq P$,
%a set of final hierarchical symbols $P_f\subseteq P$,
a call-transition relation $\cd \subseteq S \times \Sigma \times S \times P $,
an  internal-transition relation $\id \subseteq S \times \Sigma \times S $, 
and a return-transition relation $\rd \subseteq S \times P \times \Sigma \times S  $.




An NWA $\cN = (S, \Sigma, S_0, F, P, \cd, \id, \rd )$ works as follows with input a nested word $\w$. $\cN$ starts in an initial state in $S_0$ and reads $\w$ from left to
right. The state is propagated along the linear edges of $\w$ as in case of
a standard word automaton.
However, at a call position in $\w$, the nested word automaton propagates a state
along the linear edge together with a hierarchical symbol along the nesting edge of $\w$. 
At a return position in $\w$, the new state is determined based on the
state propagated along the linear edge as well as the symbol along the incoming
nesting edge.
Formally, a run $\rho$ of the automaton $\cN$ over a nested word
$\w=(a_1 \cdots a_n, \mu)$ is a sequence $s_0, s_1, \ldots, s_n$ of
states along the linear edges,
and a sequence $p_i$, for every call position $i$, of hierarchical symbols 
along the nesting edges,
such that: (a) $s_0\in S_0$; (b) for each call position $i$, it holds that $(s_{i-1},a_i,s_i,p_i)\in\cd$; (c) for each internal position $i$, it holds that $(s_{i-1},a_i,s_i)\in\id$; and (d) for each return position $i$ such that $\mu(j, i)$ holds, we have that $(s_{i-1}, p_j, a_i,s_i)\in\rd$. Moreover, the run $\rho$ is accepting if $s_n \in F$, and 
\begin{eqnarray*}
&\cL(\cN) \ = \ \{ \w \mid \w \text{ is a nested word over } \Sigma^* \text{ and there exists an accepting run of } \cN \text{ with input }\w\}.&
\end{eqnarray*}
The emptiness problem for nested word automata ask whether, given a NWA $\cN$, there exists a nested word $\w$ accepted by $\cN$. This is a fundamental problem when looking for faulty executions of a program with nested calls to subroutines; if $\cN$ is used to encode the complement of a property we expect to be satisfied by a program, then a nested word $\w \in \cL(\cN)$ encodes a bug of this program. In this sense, the following is also a very relevant problem for understanding how faulty a program~is:
%whether a program has faulty executions:
\begin{center}
	\framebox{
		\begin{tabular}{ll}
			\textbf{Problem:} &  $\snwa$\\
			\textbf{Input:} & A nested word automaton $\cN$ and a string $0^n$\\
			\textbf{Output:} & $|\{ \w \in \cL(\cN) \mid |\w| = n\}|$
		\end{tabular}
	}
\end{center}
As there exists a trivial polynomial-time parsimonious reduction from $\snfa$ to $\snwa$, we have that $\snwa$ is $\sharpp$-complete. Interestingly, from the existence of an FPRAS for $\stta$ (see Corollary \ref{cor:fpras-ta-bta}) and the results in \cite{AM09} showing how nested word automata can be represented by using tree automata over binary trees, it is possible to prove that:
\begin{theorem}
$\snwa$ admits an FPRAS
\end{theorem}


\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
\node[circ, fill=black] (a1) {};
\node[circw, below=0mm of a1] (v1) {$1$};
\node[circ, fill=black,right=10mm of a1] (a2) {}
edge[arrin] (a1);
\node[circw, below=0mm of a2] (v2) {$2$};
\node[circ, fill=black,right=10mm of a2] (a3) {}
edge[arrin] (a2);
\node[circw, below=0mm of a3] (v3) {$3$};
\node[circ, fill=black,right=10mm of a3] (a4) {}
edge[arrin, dashed, bend right, in=-135, out =-45] (a2)
edge[arrin] (a3);
\node[circw, below=0mm of a4] (v4) {$4$};
\node[circ, fill=black,right=10mm of a4] (a5) {}
edge[arrin] (a4);
\node[circw, below=0mm of a5] (v5) {$5$};
\node[circ, fill=black,right=10mm of a5] (a6) {}
edge[arrin, dashed, bend right, in=-120, out =-45] (a5)
edge[arrin] (a5);
\node[circw, below=0mm of a6] (v6) {$6$};
\node[circ, fill=black,right=10mm of a6] (a7) {}
edge[arrin, dashed, bend right, in=-135, out =-45] (a1)
edge[arrin] (a6);
\node[circw, below=0mm of a7] (v7) {$7$};
\node[circ, fill=black,right=10mm of a7] (a8) {}
edge[arrin] (a7);
\node[circw, below=0mm of a8] (v8) {$8$};
\end{tikzpicture}
\end{center}
\caption{A nested word}
\label{fig:shape}
%\end{center}
\end{figure}

\subsection{Knowledge compilation}

\input{DNNFcircuits}




==> conclusion.tex <==
\cristian{TODO: Update this conclusions to the new plan}

In this work, we provide the first polynomial time approximation algorithms for the $n$-slice of regular tree languages, and also the first polynomial time uniform samplers from this class. In addition to the recent result of \cite{Arenas19}, which provides polynomial time algorithms for the restricted class of regular languages, to the best of our knowledge this work demonstrates only the second instance of an ambiguous formal language for which an FPRAS and polynomial time sampler exist. Thus, a natural open question is which other formal languages admit efficient approximation and sampling algorithms. It would be particularly interesting to obtain negative results: namely, examples of formal languages which do not admit an FPRAS under known complexity assumptions. Such a candidate assumption would be a reduction from the problem $\#$BIS of counting the number of independent sets in a bipartite graph, which is complete for an intermediate class of counting problems for which it is unknown whether polynomial approximation algorithms exists \cite{dyer2004relative}.

One particularly interesting question is whether our results can be obtained by Monte-Carlo Markov Chain approaches. Despite being a extremely successful technique in the design of randomized approximation algorithms, so far it appears that formal languages are resistant to this approach, and do not admit any naturally convergent chains (for instance, \cite{gore1997quasi} reports a similar observation). Thus, the discovery of a quickly mixing Markov chain for tree languages, or even the subclass of regular languages, would be a highly interesting and potentially enlightening result.

==> joins-to-trees.tex <==
% !TeX spellcheck = en_US
%!TEX root = main.tex

Conjunctive queries are the most common class of queries used in
database systems, as well as the most studied in the database
literature. A conjunctive query (CQ) is constructed by combining the
join operator with a projection operator to specify the output
columns, and a selection operator to indicate that some columns must
have the same values or must have a specific value. For example,
consider a university database consisting of the following relations:
$\Und(a)$ indicates that $a$ is an undergraduate student, $\Grad(a)$
indicates that $a$ is a graduate student, $\Enr(a, b)$ indicates
student $a$ is enrolled in course $b$, and $\Course(b, c)$ indicates
course $b$ is given by department $c$. Then the following CQ is used
to retrieve the undergraduate students who are taking courses in the
Computer Science~Department:
\begin{eqnarray*}
Q_1(x) & \leftarrow & \Und(x), \Enr(x,y), \Course(y,\CS).
\end{eqnarray*}
Notice that we use the common {\em rule notation} for CQs, instead
of the equivalent form in relational algebra where the operators join
($\bowtie$), projection ($\pi$) and selection ($\sigma$) are
explicitly mentioned~\cite{DBLP:books/daglib/0020812}. In particular,
in the previous query, the relations to be joined are simply listed
separated by commas (recall that the join operator is associative, so
no parentheses need to be specified), and variables $x$, $y$ are used
to indicate values in these relations. Such variables may be shared by
two or more relations to specify that some columns must have the same
values, and they may be replaced by specific values, like \CS, to
indicate that such columns must take these values. Finally, the output
columns of the query are specified in the left-hand side of
the rule $Q_1(x)$, which in this case indicates that the values stored
in the variable $x$ must be returned by the query.

The problem of evaluating a conjunctive query has been extensively
studied, as it is of paramount importance for databases. In what
follows, we refer to the decision version of this problem, where the
task is to verify whether a tuple of values $\bar a$ is an answer to a
CQ $Q$ over a database $D$, which is denoted by $\bar a \in Q(D)$.
Starting with the work in~\cite{CM77}, where this problem is shown to
be $\np$-complete, its complexity has been extensively studied,
searching for natural restrictions that allow efficient evaluation
algorithms~\cite{Y81,CR97,GSS01,GLS02,GGLS16}, parameterized versions
of the problem that allow to improve our understanding of its
complexity~\cite{PY97,FG06,DF13}, and evaluation algorithms that are
worst-case optimal~\cite{AGM08,NPRR18}.

Beginning with the work in~\cite{Y81}, a line of research that has
been particularly fruitful in finding tractable cases for the
evaluation of CQs is based on analyzing the {\em degree of cyclicity}
of their underlying structure. For example, consider
the following CQ to retrieve the graduate students that are taking
courses both in the Computer Science and Mathematics Departments:
\begin{eqnarray}\label{eq-cq-acyclic}
Q_2(x) & \leftarrow
& \Grad(x), \Enr(x,y), \Enr(x,z), \Course(y,\CS), \Course(z,\Math).
\end{eqnarray}
This query is considered to be acyclic as it can be encoded by a {\em
join tree}, that is, by a tree $t$ where each node is labeled by the
relations occurring in the query, and which satisfies the following
connectedness property: each variable in the query induces a connected
subtree of $t$~\cite{Y81}. In particular, a join tree for query
$Q_2(x)$ is depicted in Figure \ref{fig-cq-w-aw-A}, where the
connected subtree induced by variable $x$ is marked in green (clearly,
the subtrees induced by variables $y$ and $z$ are connected as
well). An acyclic conjunctive query $Q$ can be efficiently evaluated
by using a join tree $t$ enconding it; in fact, Yannakakis'
Algorithm~\cite{Y81} computes the answers to $Q$ over a database by
traversing $t$ in a bottom-up manner, using the connectedness property
to avoid storing large intermediate results. More precisely, given an
acyclic CQ $Q$, a database $D$ and a tuple $\bar a$ of values, the
algorithm verifies whether $\bar a \in Q(D)$ in time
$O(|Q|\cdot|D|\cdot\log|D|)$.
%where $\|Q\|$ and $\|D\|$ are the
%sizes of $Q$ and $D$, respectively.
Moreover, a tree {\em witnessing} the fact that $\bar a \in Q(D)$,
where the variables occurring in $Q$ are assigned values from $D$, can
be constructed by this algorithm in this time.
%$O(|Q|\cdot|D|\cdot\log|D|)$
For example, consider again CQ $Q_2(x)$ defined
in \eqref{eq-cq-acyclic}, and assume that $\duniv$ database shown in
Figure \ref{fig-db-univ}. Then we have that $\ray$ is an answer to
$Q_2$ over $\duniv$, as $\ray$ is a graduate student who is taking courses
both in the Computer Science and Mathematics Departments. Two witness
trees for this answer, which can be generated in polynomial time by
Yannakakis' Algorithm, are shown in Figure~\ref{fig-cq-w-aw-B}. Notice
that the assignments to variable $y$ that distinguish these two trees
are marked in blue.

\begin{figure}[ht]
\begin{center}
\begin{tabular}{|c|c|cc|c|cc|}\cline{1-1} \cline{3-4} \cline{6-7} 
\Grad & \ \ \ \ \ \ \ \ \ \ & \multicolumn{2}{|c|}{\Enr} & \ \ \ \ \ \ \ \ \ \ & \multicolumn{2}{|c|}{\Course}\\\cline{1-1} \cline{3-4} \cline{6-7} 
\hill & & \hill & \cso & & \cso & \CS\\
\ray & & \ray & \cso & & \cst & \CS\\\cline{1-1}
\multicolumn{1}{c}{} & & \ray & \cst & & \matho & \Math\\\cline{6-7}
\multicolumn{1}{c}{} & & \ray & \matho & \multicolumn{2}{c}{} \\\cline{3-4}
\end{tabular}
\end{center}
\caption{A database $\duniv$ storing information about courses in a university.\label{fig-db-univ}} 
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{0.20\textwidth}
\begin{center}
\begin{tikzpicture}
\node[rect, fill=green!20] (a1) {{\footnotesize $\Grad(x)$}};
\node[rectw, below=7mm of a1] (a2) {};
\node[rect ,fill=green!20, left=2mm of a2] (a3) {{\footnotesize $\Enr(x,y)$}}
edge [thick] (a1);
\node[rect, fill=green!20, right=2mm of a2] (a4) {{\footnotesize $\Enr(x,z)$}}
edge [thick] (a1);
\node[rect, below=6mm of a3] (a5) {{\footnotesize $\Course(y,\CS)$}}
edge [thick] (a3);
\node[rect, below=6mm of a4] (a6) {{\footnotesize $\Course(z,\Math)$}}
edge [thick] (a4);
\end{tikzpicture}
\end{center}
\caption{A join tree.\label{fig-cq-w-aw-A}}
\end{subfigure}
\begin{subfigure}{0.54\textwidth}
\begin{center}
\begin{tikzpicture}
\node[rect] (wa1) {{\footnotesize $\Grad(\ray)$}};
\node[rectw, below=7mm of wa1] (wa2) {};
\node[rect, left=1mm of wa2] (wa3) {{\footnotesize \ $\Enr(\ray,{\color{blue} \cso})$}}
edge [thick] (wa1);
\node[rect, right=1mm of wa2] (wa4) {{\footnotesize $\Enr(\ray,\matho)$}}
edge [thick] (wa1);
\node[rect, below=6mm of wa3] (wa5) {{\footnotesize $\Course({\color{blue} \cso},\CS)$}}
edge [thick] (wa3);
\node[rect, below=6mm of wa4] (wa6) {{\footnotesize $\Course(\matho,\Math)$}}
edge [thick] (wa4);


\node[rect, right=28mm of wa1] (swa1) {{\footnotesize $\Grad(\ray)$}};
\node[rectw, below=7mm of swa1] (swa2) {};
\node[rect, left=1mm of swa2] (swa3) {{\footnotesize $\Enr(\ray,{\color{blue} \cst})$}}
edge [thick] (swa1);
\node[rect, right=1mm of swa2] (swa4) {{\footnotesize $\Enr(\ray,\matho)$}}
edge [thick] (swa1);
\node[rect, below=6mm of swa3] (swa5) {{\footnotesize $\Course({\color{blue} \cst},\CS)$}}
edge [thick] (swa3);
\node[rect, below=6mm of swa4] (swa6) {{\footnotesize $\Course(\matho,\Math)$}}
edge [thick] (swa4);
\end{tikzpicture}
\end{center}
\caption{Two witness trees for the answer $\ray$.\label{fig-cq-w-aw-B}}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\begin{center}
\begin{tikzpicture}
\node[rect] (awa1) {{\footnotesize $\Grad(\ray)$}};
\node[rectw, below=7mm of awa1] (awa2) {};
\node[rect, left=1mm of awa2] (awa3) {{\footnotesize $\Enr(\ray,\star)$}}
edge [thick] (awa1);
\node[rect, right=1mm of awa2] (awa4) {{\footnotesize $\Enr(\ray,\star)$}}
edge [thick] (awa1);
\node[rect, below=6mm of awa3] (awa5) {{\footnotesize $\Course(\star,\CS)$}}
edge [thick] (awa3);
\node[rect, below=6mm of awa4] (awa6) {{\footnotesize $\Course(\star,\Math)$}}
edge [thick] (awa4);
\end{tikzpicture}
\end{center}
\caption{An anonymous tree for the answer $\ray$.\label{fig-cq-w-aw-C}}
\end{subfigure}

\caption{Join, witness and anonymous trees for the acyclic CQ $Q_2(x)$ defined in \eqref{eq-cq-acyclic}.\label{fig-cq-w-aw}}
\end{figure}

In this work, we are interested in two fundamental problems that are
tightly related to conjunctive query evaluation, namely generating
uniformly and counting the answers to a conjunctive query. More
precisely, given a CQ $Q$ and a database $D$, in the latter problem we
need to compute the number of answers to $Q$ over $D$, that is
$|Q(D)|$, while in the former we need to generate, at random, a tuple
in $Q(D)$ with probability $1/|Q(D)|$. In the following paragraphs, we
explain the key role that trees play in our solutions to these
problems for acyclic CQs. For the sake of presentation, we focus on
the task of counting the number of answers to an acyclic CQ, which is
denoted by $\sacq$. The ideas presented below are also applicable to
the uniform generation task.

As a consequence of the $\np$-hardness of the evalution problem for
CQs, it is obtained that the problem of computing $|Q(D)|$, given a CQ
$Q$ and a database $D$ as input, is $\sharpp$-hard and does not admit
an FPRAS (unless $\rp = \np$). However, the previous $\np$-hadness
property is no longer valid for acyclic conjunctive queries, so it is
natural to ask whether $\sacq$ can be solved in polynomial time. In
particular, one may be tempted to think that this question has a
positive answer, given the tree structure of an acyclic CQ $Q$, the
use of witness trees to check in polynomial time whether a tuple is an
answer to $Q$ over a database, and the fact that such witness trees
can be counted in polynomial time. Unfortunately, there is no
one-to-one correspondence between the answers to an acyclic CQ and
their witness trees. As an example of this, recall that
Figure~\ref{fig-cq-w-aw-B} shows two distinct witness trees for the
same answer to the acyclic CQ defined in \eqref{eq-cq-acyclic}. Thus,
this intuition fails and, in fact, it turns
out that $\sacq$ is $\sharpp$-complete~\cite{PS13}.

One of the main goals of this paper is to construct an FPRAS for
$\sacq$, whose existence is not precluded by any previous result.  A
first observation here is that if in a witness tree $t$, only output
variables are given actual values and non-output variables are
assigned an anonymous symbol $\star$, then there will be a one-to-one
correspondance between answers to a query and witnesses. Let's us
denote such structures as {\em anonymous} trees, an example of which
is given in Figure \ref{fig-cq-w-aw-C}. But how can we specify when an
anonymous tree is valid? For example, assume that $t'$ is the
anonynomous tree obtainined by replacing $\ray$ by $\hill$ in
Figure \ref{fig-cq-w-aw-C}. Then $t'$ should not be considered as a
valid anonymous tree, given that $\hill$ is not an answer to $Q_2$
over $\duniv$ ($\hill$ is not taking any courses in the Mathematics
Department). A second observation is that the validity of an anonymous
tree can be specificied by a tree automaton. More precisely, given an
acyclic CQ $Q$ and a database $D$, it is possible to construct in
polynomial time a tree automaton $\cT$ such that for every tuple $\bar
a$ of values: $\bar a \in Q(D)$ if and only if the anonymous tree for
$\bar a$ is accepted by $\cT$. Hence, tree automata provide the right
level of abstraction to study $\sacq$, as this problem can be reduced
in polynomial time to the problem of counting the number of trees of
size $n$ accepted by a tree automaton $\cT$. In what follows, we prove
the existence of an FPRAS for this latter problem, which allows us to
conclude that $\sacq$ admits an FPRAS as well.

\marcelo{I don't think we have space to include the following figure. I leave it here just in case we want to explain in more detail how a tree automaton is constructed from an acyclic CQ and a database.}

\begin{figure}[ht]
\begin{subfigure}{0.60\textwidth}
\begin{center}
{\small\begin{tabular}{rcl} {\color{red} $\sinit \ \ \Grad(\ray)$} &
{\color{red} \ $\to$ \ } & {\color{red} $\ell_{\Enr(\ray,\cso)}\ \
r_{\Enr(\ray,\matho)}$}\\
%$\sinit \ \ \Grad(\ray)$ & \ $\to$ \ & $\ell_{\Enr(\ray,\cso)}\ \ r_{\Enr(\ray,\matho)}$\\ 
$\sinit \ \ \Grad(\hill)$ & \ $\to$ \ & $\ell_{\Enr(\hill,\cso)}\ \ r_{\Enr(\hill,\cso)}$\\
{\color{red} $\ell_{\Enr(\ray,\cso)}\ \ \Enr(\ray,\star)$} & {\color{red} \ $\to$ \ } & {\color{red} $f_{\Course(\cso,\CS)}$}\\
$\ell_{\Enr(\ray,\cst)}\ \ \Enr(\ray,\star)$ & \ $\to$ \ & $f_{\Course(\cst,\CS)}$\\
$\ell_{\Enr(\hill,\cso)}\ \ \Enr(\hill,\star)$ & \ $\to$ \ & $f_{\Course(\cso,\CS)}$\\
{\color{red} $r_{\Enr(\ray,\matho)}\ \ \Enr(\ray,\star)$} & {\color{red} \ $\to$ \ } & {\color{red} $f_{\Course(\matho,\Math)}$}\\
%$r_{\Enr(\hill,\cso)}\ \ \Enr(\hill,\star)$ & \ $\to$ \ & $f_{\Course(\cso,\Math)}$\\
{\color{red} $f_{\Course(\cso,\CS)}\ \ \Course(\star,\CS)$} & {\color{red} \ $\to$ \ } & {\color{red} $\cdot$}\\
{\color{red} $f_{\Course(\matho,\Math)}\ \ \Course(\star,\Math)$} & {\color{red} \ $\to$ \ } & {\color{red} $\cdot$}
\end{tabular}
}
\end{center}
\caption{Some of the transition rules of the automaton.\label{fig-cq-ta-A}}
\end{subfigure}
\begin{subfigure}{0.40\textwidth}
\begin{center}
\begin{tikzpicture}
\node[rect] (awa1) {{\footnotesize $\Grad(\ray)$}};
\node[rectw, below=7mm of awa1] (awa2) {};
\node[rect, left=1mm of awa2] (awa3) {{\footnotesize $\Enr(\ray,\star)$}}
edge [thick] (awa1);
\node[rect, right=1mm of awa2] (awa4) {{\footnotesize $\Enr(\ray,\star)$}}
edge [thick] (awa1);
\node[rect, below=6mm of awa3] (awa5) {{\footnotesize $\Course(\star,\CS)$}}
edge [thick] (awa3);
\node[rect, below=6mm of awa4] (awa6) {{\footnotesize $\Course(\star,\Math)$}}
edge [thick] (awa4);


\node[above left=-2mm of awa1] {{\color{red} {\footnotesize $\sinit$}}}; 
\node[above left=-2mm of awa3] {{\color{red} {\footnotesize $\ell_{\Enr(\ray,\cso)}$}}}; 
\node[above right=-2mm of awa4] {{\color{red} {\footnotesize $r_{\Enr(\ray,\matho)}$}}}; 
\node[above left=-2mm of awa5] {{\color{red} {\footnotesize $f_{\Course(\cso,\CS)}$}}}; 
\node[above right=-2mm of awa6] {{\color{red} {\footnotesize $f_{\Course(\matho,\Math)}$}}}; 
\end{tikzpicture}
\end{center}
\caption{A run of the automaton on the anonymous tree from Figure \ref{fig-cq-w-aw-C}.\label{fig-cq-ta-B}}
\end{subfigure}

\caption{Some transition rules and a run of the tree automaton generated from acyclic CQ $Q_2(x)$ defined in \eqref{eq-cq-acyclic} and database $\duniv$ in Figure \ref{fig-db-univ}.\label{fig-cq-ta}}

\end{figure}






